AQUA: Network-Accelerated Memory Offloading for LLMs in Scale-Up GPU Domains

Inference on large-language models (LLMs) is constrained by GPU memory capacity. A sudden increase in the number of inference requests to a cloud-hosted LLM can deplete GPU memory, leading to contention between multiple prompts for limited resources. Modern LLM serving engines deal with the challenge of limited GPU memory using admission control, which causes them to be unresponsive during request bursts. We propose that preemptive scheduling of prompts in time slices is essential for ensuring responsive LLM inference, especially under conditions of high load and limited GPU memory. However, preempting prompt inference incurs a high paging overhead, which reduces inference throughput. We present Aqua, a GPU memory management framework that significantly reduces the overhead of paging inference state, achieving both responsive and high-throughput inference even under bursty request patterns. We evaluate Aqua by hosting several state-of-the-art large generative ML models of different modalities on servers with 8 Nvidia H100 80G GPUs. Aqua improves the responsiveness of LLM inference by 20X compared to the state-of-the-art and improves LLM inference throughput over a single long prompt by 4X.

==> tex/design-bait.tex <==
\section{\sysname design}

\sysname decouples the hardware resource allocation on the GPU into memory and compute and allocates unused memory to other memory constrained workloads on GPUs to efficiently handle bursts and improves the performance of workloads. 
\sysname has three main components \sysnameprofiler, \sysnamelib and \sysnamePl. \sysnameprofiler(\S~\ref{sec:opportunity}) is a framework to systematically evaluate the available free memory on a GPU. \sysnamelib is an inter-GPU memory-management library that interfaces with the popular ML framework, PyTorch~\cite{pytorch}. \sysnamelib transparently offloads tensors to available free memory on GPUs connected over a fast inter-GPU network. \sysnamePl is a model placement algorithm that optimally maps ML models to GPUs in a cluster to maximize opportunities of offloading free GPU memory using \sysnamelib
 
\begin{figure}[h]
    \centering
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\columnwidth]{plots/bait/aqua_tpt.pdf}
        \caption{\small OPT-30B}
        \label{fig:flexgen_bait}
    \end{subfigure}
    \begin{subfigure}[b]{0.18\textwidth}
        \includegraphics[width=\columnwidth]{plots/bait/link_tpt.pdf}
        \caption{\small Bandwidth}
        \label{fig:link_bait}
    \end{subfigure}
    \caption{\small Figure~\ref{fig:flexgen_bait} shows OPT-30B and a prompt of 8192 tokens are too large for a single A100 80 GB GPU. So, the throughput on a single GPU is zero. The current state of the art enables inference on large models and prompts by swapping to DRAM over PCIe. \sysname can improve the throughput by $6X$ by transparently storing the swap space on a neighboring GPU over \nvlinks which is an order of magnitude faster than PCIe. Figure~\ref{fig:link_bait} shows the disparity between the bandwidths of \nvlinks vs PCIe across generations.}
    \label{fig:bait}
\end{figure}

% % Spatial prefetching does not cut it in traditional paging
% % Page faults happen in critical path and increase the latency.

% \myparab{What about scaling out?}
% Tell you need a lot of \$ for this. Focus on the performance of individual instance of the model deployment. For batch workloads and offline workloads, scaling out doesn't matter anyway because the traffic is constant. We are aiming to minimize the resources required by maximizing resource utilization. For interactive workloads that depend on traffic, we provide a way to increase the sustainable traffic rate by still being responsive by up-to some \%.

\myparab{Why offload memory to an interconnected GPU?}
We demonstrate the benefits of preempting to neighboring GPU memory over \nvlinks in Figure~\ref{fig:bait}. A 30 billion parameter model on an A100 GPU with 80 GB of memory fails to infer a 8192-token prompt due to memory constraints. State of the art research prototypes~\cite{flexgen,hetegen2024} overcome this challenge by swapping the inference context of the next layer while overlapping it with the compute of current layer but achieve only 2 tokens/second. The throughput improves to 8 tokens per second with just 10 gigabytes of swap space on a neighboring GPU. This is because the workload is bottlenecked by the bandwidth between GPU and the swap space and \nvlinks has an order of magnitude higher bandwidth compared to PCIe as shown in Figure~\ref{fig:link_bait}. With NVIDIA's latest announcement of the NVL72~\cite{b200_dgx} that can connect up to 72 GPUs over \nvlinks, there will be more opportunities to leverage underutilized memory across GPUs.


\myparab{Why is this new?} 
Current resource allocators for GPUs achieve high resource utilization and goodput by multiplexing two or more models on the same GPU. Some allocators~\cite{alpa_serve,gandiva} determine the compute utilization at run time based on the traffic rate and multiplex models with higher request rates with models executing on GPUs with underutilized compute. Other allocators rely on the memory utilization in addition to compute utilization~\cite{usher} to determine the placement of models across GPUs to maximize resource utilization. However, all these allocators \emph{tightly couple} compute and memory during multiplexing multiple models, \ie it is impossible to exploit the underutilized memory on a GPU without also utilizing its compute resources. This precludes memory constrained workloads benefitting from the underutilized memory on a GPU whose compute is saturated by the workload on that GPU. Such opportunities are ample in the new generative AI space as we show in \S~\ref{sec:opportunity}.


TODO: Show graph where the CPU utilization of a GPU is 100\% while having free memory. Use stable diffusion 3 for this. Cite the ATC paper.

\myparab{What about faster GPU-DRAM interconnects?}
NVIDIA recently announced chip-to-chip \nvlinks between B200 GPUs and the DRAM in their new Grace-hopper superchip~\cite{nvidia_grace_hopper} which offers the same high speed \nvlinks bandwidth between GPUs and DRAM. While this chip enables high speed GPU to DRAM communication, there is a need for faster preemption system for two reasons. First, organizations have already invested heavily on the current state of the art GPUs, \eg Meta is spending billions of dollars to acquire 100s of thousands of H100 GPUs~\cite{meta_nvidia_h100_purchases,zuck_reel} and these DGXes will continue to exist alongside newer hardware. Second, NVIDIA has also announced a traditional DGX~\cite{b200_datasheet} with their B200 GPUs without the chip-to-chip interconnect between GPUs and DRAM whose clusters will necessitate systems like \sysname for memory constrained workloads. 


==> tex/introduction.tex <==
\section{Introduction}

% Recent years have seen the explosive growth in popularity
% of large machine learning (ML) models\ga{cite}. End users are leveraging 
% large ML models to improve their efficiency on a multitude of 
% tasks ranging from summarization to multimedia content
% creation\cite{openai_customer_stories,azure_openai_blog,
% aws_generative_ai_use_cases,mewtant_2024}. To meet consumer demands, cloud providers
% offer GPUs to rent, enabling 
% clients to run inference on pre-trained models without 
% incurring the cost overhead of deploying their own ML 
% accelerators\cite{amazon-sagemaker,azure-ai-studio,together_ai,openai-api}. 

% Renting enough GPUs for Large Language Models (LLMs) is challenging in budget 
% constrained scenarios since modern LLMs have a massive memory footprint, 
% \eg Llama-405B requires 800 gigabytes just to host the model\ga{do we have an example of cost? something that can strengten a bit the argument. Would be cool if we could say something like: For example, using state-of-the-art model on XYX would cost...}. Moreover, inference on LLMs generates and uses inference context~\cite{attention} which can take several gigabytes of additional GPU memory. The high memory capacity requirement, combined with limited GPU resources, leads to a memory capacity bottleneck that causes unresponsiveness and starvation\ga{cite}.

% From the perspective of a cloud operator, providing
% \emph{inference-as-a-service} on modern generative ML models 
% poses a challenging resource allocation problem. Modern 
% generative ML models have a massive memory footprint~\cite{llama,codellama,mistral,mixtral,mpt}. 
% For example, GPT-4 is a transformer-based generative 
% language model with roughly two trillion parameters~\cite{mtnlg}.
% In such cases, the model parameters themselves can consume 
% majority of the available high-bandwidth memory (HBM) of ML accelerators.
% Moreover, inference on large language models (LLMs) generates 
% and uses inference context, including a key-value cache~\cite{attention} 
% which can take several gigabytes of GPU memory. While 

% \begin{figure}[h]
%     \centering
%     \begin{subfigure}[b]{0.23\textwidth}
%     \includegraphics[width=\columnwidth]{plots/cfs-mb/cfs_micro_ttfts.pdf}
%     \caption{\small TTFTs}
%     \label{fig:cfs_mb_ttft}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.23\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{plots/cfs-mb/cfs_micro_latencies.pdf}
%     \caption{\small RCT}
%     \label{fig:cfs_mb_rct}
%     \end{subfigure}
%     \caption{\small Responsiveness (measured using time-to-first-token or TTFT) and 
%     throughput (measured using request completion time or RCT) of inference queries on LLMs. 
%     Since vLLM batch processes queries, it has low RCT (high throughput) 
%     but high TTFT (low responsiveness). Fair-scheduling queries improves 
%     responsiveness but paging overheads dominate RCT. \sysname reduces 
%     paging overheads by offloading memory over high-speed multi-GPU 
%     interconnects (\eg \nvlinks), achieving responsive inference with 
%     low RCT.}
%     \label{fig:cfs_mb}
% \end{figure}

% % what is the problem?
% \myparab{Memory capacity bottleneck.} 
% \ga{this starts as a sort of repetition of the previous}LLM inference is bottlenecked by memory capacity. LLMs use the attention mechanism~\cite{attention} to process the input prompts by breaking them into tokens and generating key and value vectors for each token, stored in a key-value (kv) cache. This cache grows with the input and generated sequence length, requiring additional memory beyond the model weights~\cite{vllm} and insufficient GPU memory often referred to as High Bandwidth Memory (HBM) leads to memory contention across input prompts. Provisioning additional memory to alleviate the contention can be costly and impractical for organizations with budget constraints because GPUs tightly couple compute and memory hardware, making it challenging to increase the memory capacity of a server without adding more GPUs. We refer to memory capacity contention when we mention memory contention in the rest of the paper.

% How does it affect LLM serving?
% \myparab{Memory contention causes unresponsiveness.} 
% Memory contention causes certain prompts to be queued leading to temporary 
% unresponsiveness due to head of line blocking. Serving engines focus on optimizing
% throughput and device utilization and employ a First-Come, First-Served (FCFS) 
% scheduling policy~\cite{vllm,fcfs_fairness}, admitting new prompts only when there 
% is enough GPU memory. As a result, prompts that are waiting will be unresponsive. 
% This approach is in stark contrast with traditional operating 
% systems\ga{i understand what you mean but it sounds weird the way you wrote. 
% I might think: why shall I worry in being in stark constrast with OS design?}, which use preemptive scheduling for equitable job progression, such as the Linux Completely Fair Scheduler (CFS)~\cite{linux_cfs}. If we want to apply this to LLMs for achieving fair responsiveness across users, it is essential to multiplex the GPU's compute by preemptively paging the inference context of promtps between the GPU and DRAM. 


% What do current systems do?

% What are we doing?
\myparab{Finding faster memory outside GPU.} 
GPU providers such as Nvidia design servers with multiple GPUs, 
each equipped with diverse hardware resources and interconnected 
through complex heterogeneous links (e.g., PCIe, \nvlinks). 
Not all the workloads fully utilize the allocated resources, 
leading to underutilization of certain resources while the same 
resources become bottlenecks for other workloads. For instance, 
some workloads underutilize HBM capacity while HBM is a critical 
bottleneck for others. 

\myparab{Key Insight}: 
We argue for the decoupled allocation of resources on GPUs, 
a strategy that will improve resource utilization and significantly 
boost application performance. Specifically, we show that the HBM 
capacity on a GPU is underutilized by certain workloads and how 
using this spare capacity for paging improves the performance of 
other workloads. This spare memory is accessible over \nvlinks 
at a much faster rate compared to PCIe and when allocated to 
a workload on an interconnected GPU, it significantly improves 
the paging performance and end-to-end application performance. 
As the size of the \nvlinks domain increases, \eg 72 GPUs in 
the Blackwell architecture, there will be more opportunities for 
decoupled hardware allocation.

% Why are existing solutions not enough?
\myparab{Current resource allocators tightly couple allocation.} 
Cloud providers build clusters using state of the art 
servers~\cite{h100_dgx} and allocate resources on these 
clusters to workloads of tenants at the GPU granularity where compute, memory and the interconnect are tightly coupled, resulting in each workload receiving all the resources. To the best of our knowledge, existing research on efficiently sharing GPUs~\cite{usher,alpa_serve,gandiva} all necessitate sharing both compute and HBM capacity on a GPU across workloads. Such approaches preclude the possibility of allocating unused memory on a GPU whose workload is fully utilizing the compute, to workloads on other GPUs. This is because sharing the unused memory also inevitable shares the saturated compute which leads to resource contention and significantly impacts the performance SLA.

% Why is doing this hard?
\myparab{Challenges.}
Accelerating memory offloads during inference on 
multi-GPU servers is challenging in practice. Our early 
experiments revealed that naively offloading context tensors 
to neighboring GPUs over \nvlinks does not provide
a speedup over offloads to DRAM since \nvlinks achieve
their advertised bandwidth only when data transfers are 
sufficiently large. Second, there is no guarantee 
that GPUs on a server will have free memory available to 
offer to memory-constrained GPUs. Unlike the abundant 
host DRAM, GPU memory is a precious resource that 
may already be in use by other inference workloads. Even if spare 
memory is available on a nearby GPU, ML models lack a mechanism 
to seamlessly access this memory without needing interference 
from the ML engineer. Third, inference workloads can change 
over time which means both the demand and supply of GPU 
memory during inference is elastic. This dynamic environment 
makes it hard to offload context to a different GPU that may 
require the memory back when it experiences high load of 
inference queries.

% \myparab{Contributions:} Discuss what to put here later.
% Cite HOL blocking paper.


% Cut text
% The memory bottleneck in these resource constrained scenarios necessitates paging to slower storage locations such as DRAM for fair and responsive inference.
% This approach contrasts with traditional operating systems, which use preemptive scheduling to ensure equitable job progression, such as the Linux Completely Fair Scheduler (CFS)~\cite{linux_cfs}. To achieve fairness across users, it is essential to multiplex the GPU's compute resources by preempting prompts from the GPU.
% 
% For instance, a doctor examining a patient's history during a visit might have many questions about the context in the history. Instead of re-computing the inference-context of the history for every new question, the engines cache the inference-context for future use. 

% In the past two years, there has been a significant surge in generative AI research, leading to its widespread use across various modalities~\cite{azure-ai-studio,aws_generative_ai_use_cases,openai_customer_stories,amazon-sagemaker}. Each model architecture benefits from distinct hardware resources. For instance, convolution layers in diffusion models benefit from faster compute cores, while transformers necessitate high-bandwidth memory (HBM)~\cite{sarathi_serve} due to the billions of weights accessed to generate each token. LLMs demand extensive memory capacity to generate responses for multiple users, and distributed LLMs require high-speed GPU-to-GPU interconnect bandwidth. Consequently, 
%In state-of-the-art servers, GPUs are interconnected using \nvlinks, which provide an order of magnitude higher bandwidth than PCIe. 

==> tex/motivation.tex <==
\section{Infrastructure for distributed ML}
\label{sec:motivation}

ML inference tasks are gaining popularity as organizations 
incorporate them into their operational processes\ga{cite}. 
State-of-the-art ML models are capable of generating a variety 
of media, like text~\cite{llama}, images~\cite{stablediffusion} 
and audio~\cite{audiogen}. Large Language Models (LLMs), a 
subset of these generative ML models, are particularly popular 
for their text generation capabilities and are extensively used in 
applications like text summarization, chatbots, and code generation. 
Organizations typically utilize hosted AI models from API 
providers like OpenAI~\cite{openai-api}, Anthropic~\cite{anthropic_claude} \etc. 
However, many organizations in regulated industries such as legal, 
medical, financial \etc, unwilling to share their enterprise data 
with other companies resort to dedicated hosting where AI models
 are hosted on cloud providers~\cite{amazon-sagemaker,azure-ai-studio,together_ai}. 
 his is better for organizations focused on other goals because 
 buying and operating state-of-the-art GPUs is expensive in 
 terms of cost and effort. 
% Organizations own servers or they rent servers. based on if they are a regulated industry or not.
% Describe the servers: GPUs, used for distributed serving because models are large. So, you need nvlinks.

\myparab{LLMs have memory contention.} 
LLMs convert the inference query text, called a \emph{prompt}, 
into tokens. A multi-dimensional vector, called the embedding vector, 
represents different aspects of a token's meaning~\cite{word2vec,bert}. 
Embeddings of tokens in the prompt are input to the LLM during 
inference. The high accuracy of LLMs on downstream tasks is 
attributed to their transformer-based model architecture that 
relies on the attention mechanism\cite{attention}. The attention 
mechanism~\cite{attention} calculates \emph{key and value vectors} for 
every token of the prompt in every transformer layer of the LLM. The 
key and value vectors of all the previous tokens are required to
 generate the subsequent token. So, the serving engines cache 
 the key and value vectors (kv cache) which grows with the size 
 of the prompt and the generated text. \textbf{Takeaway 1: } 
 \emph{To execute inference on LLMs, additional memory is 
 needed to store inference context beyond just storing the model weights.} 

% Organizations operate on a budget constraint and run multiple models on the same infrastructure. LLMs for agents, chatbots, offline workloads, image generation, audio generation etc.
% Some of these systems need to page:
\myparab{Budget constraints lead to memory contention.} 
Renting a GPU server on the cloud is expensive which often 
leads to memory contention. For instance, a single H100 GPU on 
AWS, Azure, or GCP costs at least \$10 per hour~\cite{gcp_h100_pricing,aws_h100_pricing}. 
Consequently, organizations are forced to operate within budget 
constraints while accommodating their diverse generative AI needs, 
including chatbots, agents, and offline workloads such as summarization, 
classification, and image/audio generation. Even with a budget 
for enough GPUs to accommodate the model weights, LLMs need additional 
memory to store the inference context (kv cache) for accurate token 
prediction (Takeaway 1) and limited additional GPU memory capacity 
leads to memory contention. As memory contention causes 
unresponsiveness and starvation and adding memory to the 
deployment is expensive because of cloud schedulers allocating
 hardware at the GPU granularity, LLM serving is left with the 
 only choice of paging between GPU and DRAM~\cite{flexgen,hetegen2024,
 llama31_blog} to increase the capacity. 

% Paging to avoid starvation.
% Large models 70B, 405B, 30B models etc are good at summarization, sentiment analysis, chain of though and other batch workloads which are not latency critical and hence can run in resource constrained environments. Paging is a good use case here.
\myparab{Paging to avoid starvation.} 
Large models necessitate paging to avoid starvation. Many open 
source models like Llama-70B, Llama-405B~\cite{llama}, 
OPT-30B~\cite{opt-30b} \etc, have shown state-of-the-art performance 
in tasks such as summarization, sentiment analysis and classification. 
Such tasks can tolerate higher latencies and are executed in batch 
with a lower SLA guarantee, \eg OpenAI offers a batch API with 
an SLA of 24 hours~\cite{openai_batch} at a significantly lower 
price. The input prompts for these tasks are long, necessitating 
a large amount of memory in addition to the considerable number 
of model weights, which can exceed the GPU budget and organizations 
often face challenges in leveraging these models effectively. 

Even when GPUs are available, there may be insufficient capacity 
to load both the model weights and the inference context and 
the inference stalls without enough capacity leading to 
starvation of prompts. Academic and open source systems~\cite{llama31_blog} 
are addressing the starvation by paging model weights and the 
inference context to the DRAM and loading them on demand 
to the GPU on a layer by layer basis. These systems have 
also optimized the loading latency by overlapping 
communication with compute~\cite{flexgen}.

% Paging for responsiveness.
% Users are directed to chatbots if people are all busy and it can be very frustrating if the chatbot is also busy and the users need to wait 10s of seconds to receive response. Trade off TTFT for TPOT. as long as it is near human-reading speed, it is okay.
% Tradeoff performance for responsiveness and fairness. For example, customer service agents. 
% Prompt caching for latency sensitive scenarios. Loading them in DRAM can lead to 3x more latency. Google many shot in context learning.
\myparab{Paging for responsiveness.} 
Unresponsiveness in latency-sensitive scenarios, 
such as chatbots necessitates paging. State-of-the-art LLM 
serving engines typically use a First Come, First Serve (FCFS) 
scheduling approach, admitting new prompts into the GPUs 
until memory is full. When memory is full, subsequent prompts are 
queued. This ensures quick response generation once a prompt is
 admitted, resulting in low time per output token (TPOT). However, it 
 also leads to a high time to first token (TTFT) for queued prompts,
  causing unresponsiveness. While horizontal scaling by over provisioning 
  addresses the head of line blocking issue, it is impractical in 
  budget constrained scenarios especially when the bursts are short lived.

High TTFT is undesirable, especially when users expect quick attention, \
eg many companies redirect users to chatbots when customer 
service agents are occupied~\cite{call_center}. In such situations, 
users expect low TTFT to avoid long waiting periods, as the primary 
purpose of chatbots is to reduce wait times and it is preferable to 
trade off a lower TTFT for a higher TPOT, as long as the generation 
speed remains close to human-readable speed. Traditional operating 
systems address similar resource contention issues using preemptive 
scheduling algorithms like the Linux fair scheduler~\cite{linux_cfs}. 
Adopting a similar approach for LLM serving engines requires paging
 inference contexts to DRAM, allowing the system to handle more 
 prompts than GPU memory alone can accommodate.

\myparab{Paging to enable optimizations.}
Caching optimizations in LLMs need paging to provide benefits. 
Recent advancements in LLMs, such as Google's Gemini, 
now support large prompts reaching up to one million tokens. 
Foundational language models like GPT and Llama are typically 
trained on broadly available data and are not fine-tuned 
for specific tasks. Fine-tuning these large models for multiple 
tasks can be prohibitively expensive. Recent research has shown 
that providing sufficient examples of a task within the prompt 
can enable the model to perform as if it were fine-tuned for 
that specific task~\cite{manyshot_gemini,multimodal_manyshot}, 
without the need for additional fine-tuning resources. For instance, 
including many examples of translation pairs in a rarely encountered 
language can enable the model to achieve reasonable accuracy in 
translation tasks~\cite{manyshot_gemini}. 

Despite its advantages, the repetitive processing of long prompts is computationally expensive and leads to a high TTFT. To avoid expensive re-computation, LLM providers have introduced caching the inference context associated with long prefixes for reuse across different prompts.~\cite{anthropic_caching,google_gemini}. The serving engine can skip the inference context computation of the prefix and directly start inferring on the remaining suffix which is typically small, \eg a sentence that needs to be translated. However, storing the prefix's inference context on the GPU is impractical because of its large memory footprint as the GPU needs to infer newer unrelated prompts between prompts related to the cached context. So, paging the inference context to the DRAM is essential for maintaining cache benefits. 

\subsection{Paging is slow, how to make it fast?}

As we described previously, paging is a critical mechanism especially in budget constrained scenarios to avoid unresponsiveness and starvation but the current paging data path is slow and leads to degraded performance. Today's inference serving systems are forced to offload context once inference queries exhaust the GPU HBM~\cite{flexgen,hetegen2024,llama31_blog}. The overheads of transferring context from GPU memory to the host DRAM and vice versa are high due to the limitations of PCIe bandwidth~\cite{pcie,hostcongestion}. The performance of the workloads relying on paging is severely degraded because the GPUs are idle while they wait for loading the paged data from DRAM to the GPU. The performance of workloads that page will drastically improve if we offload the data to a storage location that is accessible at an order of magnitude faster bandwidth compared to PCIe. We will first describe the hardware architecture of modern ML servers and then delineate our key insight that unlocks the potential to find such storage.

\myparab{Server targets for hosted ML.}
As LLM sizes are growing, it is infeasible to host some of them (Llama-70 B) on a single GPU and it is common practice to split the model across multiple GPUs during inference~\cite{megatron}. To address this need efficiently, server-scale multi-accelerator systems (\eg Nvidia DGX~\cite{dgx}, Cerebras WSE~\cite{cerebras}, Intel Gaudi~\cite{gaudi}) have become building blocks of datacenter deployments. A server-scale multi-accelerator system consists of a handful of ML accelerators, connected with high-speed on-board electrical interconnects (\eg Nvidia NVlink, Google ICI) that support up to hundreds of gigabytes per second of bandwidth between pairs of accelerators. Cloud operators connect racks of server-scale multi-accelerator systems into datacenter-scale deployments using a network fabric~\cite{googletpuv4,jupiter-evolving}. \textbf{Takeaway 2: } \emph{Accelerators on multi-accelerator systems are connected at high-bandwidths of hundreds of gigabytes per second.}

\myparab{Opportunity in the modern hardware.}
We demonstrate that decoupling the allocation of hardware components within a GPU unlocks opportunities for faster paging. A GPU is increasingly looking similar to a traditional server since it has compute cores, high bandwidth memory, networking links (\nvlinks~\cite{nvlink}, ICI~\cite{googletpuv4}) similar to the CPU cores, memory on NUMA nodes and NICs on a traditional server. Workloads deployed on traditional cloud have diverse hardware requirements and cloud providers are able to efficiently utilize the resources on a traditional server by carving out individual hardware components and packaging them as virtual machines with different properties tailored to the requirements. For example, cloud providers offer compute optimized, memory optimized and storage optimized virtual machines~\cite{aws_vm_types,azure_vm_types}.

\myparab{Key insight: } 
Viewing GPUs as a server unlocks the potential to decouple the allocation of hardware resources on a GPU. Similar to traditional workloads, generative AI workloads also have a diverse hardware requirement within a multi-GPU server. For instance, convolution layers in diffusion models benefit from faster compute cores, while transformers necessitate high-bandwidth memory (HBM)~\cite{sarathi_serve} due to the billions of weights accessed to generate each token. LLMs demand extensive memory capacity to handle multiple prompts, and distributed LLMs require high-speed GPU-to-GPU interconnect. We show with experimental evidence that allocating resources at a GPU granularity leads to GPU HBM underutilization on certain workloads while other workloads are bottlenecked by the same resource. We can improve resource utilization and application performance by allocating the unused memory to a workload that needs to page memory. Since this memory can be accessed over \nvlinks at a much higher bandwidth (Takeaway 2), the performance of the paging workload significantly improves. 

% High TTFT is undesirable, especially when users expect quick attention, \eg many companies redirect users to chatbots when customer service agents are occupied~\cite{call_center}. 
\myparab{Producer consumer abstraction.}
As a first step in the decoupling direction, we decouple the allocation of memory from the remaining GPU resources. We call the workloads that need to page as consumers and workloads that have memory to offer as producers. We will experimentally demonstrate how to determine whether a workload is a producer and how much memory it has to offer in \S\ref{sec:opportunity}. 

% We call them consumers.
% Some of the workloads have memory to spare: we call them producers. 
% we characterize workloads and build a framework to measure spare memory capacity.
% Subsection: Opportunity to offload.


